A Study of Pulsation properties of 57 Non-Blazhko effect ab-type RR Lyrae stars with homogeneous metallicities from the LAMOST-Kepler/K2 survey

Homogeneous metallicities and continuous high-precision light curves play key roles in studying the pulsation properties of RR Lyrae stars. By cross-matching with LAMOST DR6, we have determined 7 and 50 Non-Blazhko RRab stars in the Kepler and K2 fields, respectively, who have homogeneous metallicities determined from low-resolution spectra of the LAMOST-Kepler/K2 project. The Fourier Decomposition method is applied to the light curves of these stars provided by the Kepler space based telescope to determine the fundamental pulsation periods and the pulsation parameters. The calculated amplitude ratios of R21, R31 and the phase differences of {\phi}21, {\phi}31 are consistent with the parameters of the RRab stars in both the Globular Clusters and the Large Magellanic Cloud. We find a linear relationship between the phase differences {\phi}21 and {\phi}31, which is in good agreement with the results in previous literature. As far as the amplitude, we find that the amplitude of primary frequency A1 and the total amplitude Atot follow either a cubic or linear relationship. For the rise time RT, we do not find its relevance with the period of the fundamental pulsation mode P1, or Atot and {\phi}21. However, it might follow a linear relationship with R31. Based on the homogeneous metallicities, we have derived a new calibration formula for the relationship of period-{\phi}31-[Fe/H], which agrees well with the previous studies.

==> referencestar.tex <==
1 &  &  &  &  \\
2 &  &  &  &  \\
3 &  &  &  &   \\
